An Empirical Study on Governance in Bitcoin's Consensus Evolution

Blockchain systems run consensus rules as code to agree on the state of the distributed ledger and secure the network. Changing these rules can be risky and challenging. In addition, it can often be controversial and take much effort to make all the necessary participants agree to adopt a change. Arguably, Bitcoin has seen centralisation tendencies in pools and in development. However, how these tendencies influence blockchain governance has received minimal community and academic attention. Our study analyses the governmental structures in a blockchain by looking into the history of Bitcoin. We investigate the process of changing consensus rules through a grounded theory analysis comprising quantitative and qualitative data from 34 consensus forks in Bitcoin and Bitcoin Cash. The results reveal the decentralised behaviour in Bitcoin and blockchain. Our results are in contrast to related work, emphasising centralisation among miners and developers. Furthermore, our results show how the consensus-driven deployment techniques and governance of consensus rules are intertwined.

==> sections/futureWork.tex <==
\section{Future work} \label{future}

Our research and analysis indicate that pool and developer centralisation are insignificant regarding the governance of permissionless blockchains.
Instead, analysing hash power distribution among individual miners could be more interesting. A better understanding of hash power distribution can reveal how many mining actors would need to collude to have longitudinal influence over a blockchain in terms of majority attacks and reduction forks. Other factors such as juristical or geographical distribution of hash power could, for instance, demonstrate how much influence governments and regulators could have in the long term.

It would also be interesting to see the frequency of miners changing between pools and whether that is related to pools' stance regarding consensus governance. That can reveal to what extent miners are exercising their governmental influence.
Furthermore, the centralisation of economic funds among users can be a factor in centralised influence over the system. If only a few actors are responsible for a large portion of the transactions and network fees, these will have considerable influence on a blockchain. Further work can provide novel contributions by finding factors that could provide insights and measure governance centralisation in blockchain systems.


==> sections/relatedWork.tex <==
\section{Related work}
\label{relatedWork}

\subsection{Bitcoin maintenance and evolution}
%Some articles on the topic of blockchain are related to this study
Several studies have investigated Bitcoin maintenance and evolution. However, those looking at Bitcoin mainly consider the governance structures and politics of the system~\cite{andersen2017patterns,de2016invisible} and the economics therein~\cite{kroll2013economics}.
The formal processes and technical approaches to perform rule changes in Bitcoin and blockchain has not been considered. 
%However, these papers can prove useful to understand how governance and politics affect the choice of the evolutionary path.

\subsection{Consequences of a chain split}
Kiffer, et al.~\cite{kiffer2017stick} provide one approach to analyse the consequences of a chain split as it evaluates the event of the Decentralized Autonomous Organization (DAO) hack in Ethereum.
They present how quantitative data from traffic on the blockchain can be analysed to understand the consequences of such an incident.
However, they did not focus on investigating the causes of failure and techniques for the evolution of consensus rules. 
%, a more comprehensive qualitative analysis is conducted in this study.

\subsection{Abortable consensus}
ADAPT (adaptive abortable BFT system) describes a dynamic switching mechanism for BFT protocols. The mechanism will cause the system to switch consensus protocol whenever the system fails or can gain some performance~\cite{chen2007abortable,guerraoui2010next,bahsoun2015making}.
The abortable consensus is designed for asynchronous systems and will prioritize progress over agreement when nodes are hard to reach. This is slightly different from the synchronous Bitcoin proof of work consensus protocol~\cite{knudsen2021consensus}.
In contrast, Bitcoin nodes must be up-to-date and in agreement for the system to be reliable. Thus, the nodes that cannot keep in sync with Bitcoin will not be able to produce blocks or provide full validation of transactions.
Additionally, as the system aborts to a different consensus protocol, it changes the system's fault tolerance. Bitcoin's strict security requirements do not allow for losing the fault tolerance of 50\%, nor is it likely to be increased.

%Bitcoin cannot afford disagreement

%These conditions are to decide when to switch are different from Bitcoin as it relies on consensus to decide when to switch. 

%This is an optimization of BFT protocols that switches between protocols as a tradeoff between agreement and progress. 

%The feature of optimization could be applicable to blockchain, and can be compared to the difficulty switching algorithm in Bitcoin.

%APADT consists of three parts: A BFT system managing and switching between predefined  However, this kind of switch requires the code for the target protocol to be implemented in all nodes before switching, which is not the case for arbitrary consensus rule changes. 

%Neiher does ADAPT consider compatability of the validity domain of the systems shared data store, which can be less strict in a ledger-less BFT system.

%The switch time in ADAPT is also decided by the primary replica running a quality control system. The main drawback with this method is that the primary replica serves as a centralized control and a single point of failure. %Something that cannot be accepted in mission critical systems such as cryptocurrencies. 

%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7161576

%The next 700 BFT

%OSS???

%http://www.infosecon.net/workshop/downloads/2013/pdf/The_Economics_of_Bitcoin_Mining,_or_Bitcoin_in_the_Presence_of_Adversaries.pdf
%Our analysis supports and deviates from this paper in the sense that devs are defacto leaders - untill there are internal conflict or external competitors.


%List and summarize
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9258860
%https://ieeexplore.ieee.org/abstract/document/8326513
%https://papers.ssrn.com/sol3/papers.cfm?abstract_id=2407834
%http://www.ledgerjournal.org/ojs/ledger/article/view/96
%https://ieeexplore.ieee.org/abstract/document/8835333

\subsection{Open source software evolution}

Research on software evolution in Open Source Software (OSS) has been conducted with different perspectives and goals.
For instance, some choose to look at the evolution of the software code itself in terms of complexity and adaptability~\cite{tu2000evolution,israeli2010linux}. 
Guzzi, et al.~\cite{guzzi2013communication} analyse what kind of discussions email lists are used for and by whom. 
Sharma, et al.~\cite{sharma2021extracting} look at these kinds of sources to understand the rationale for decisions made to accept or reject proposals in Python. 
The processes in Python resemble some similarities to Bitcoin and blockchain. However, the difference is that blockchain has different stakeholders, decision-making power structures, and requirements for consensus. 
Where Bitcoin has different roles, such as miners and validators, decentralised decision-making power structure, and the network must be in consensus for a change to be deployed, it is not a decision to be made solely by code maintainers.
% TODO: Can be added to discussion: On the contrary, our study looks at specific topics from different sources. 

\subsection{Network protocol evolution}
Holz, et al.~\cite{holz2020tracking} studied the runtime evolution and adaption of the TLS1.3 protocol. In their case, the research looked at the adoption rate and explained its nature. The transport layer protocols can be adopted at an arbitrary rate and downgraded when required in individual peer-to-peer connections. On the other hand, a blockchain rule change cannot be adopted at an arbitrary rate and must run network-wide compatible versions to prevent failure. The deployment of transport layer protocols and consensus protocols is different, although the adoption rate may act similarly as forks often are adopted over time.


==> sections/results/governance.old.tex <==
\subsection{The relationship between governance process and the level of controversy of a change}
\label{governance}

The analytical codes related to the social/political category (figure \ref{fig:codesCategories}) show how the governance process relies on the controversy of a change. A change with low controversy requires low effort in terms of agreement and deployment.
Centralisation tendencies in development and mining operations can streamline the deployment of non-controversial changes.
Changes that can be deployed most quickly are related to fixing an immediate issue in the blockchain. In that case, the developers are in a hurry to implement a solution while miners and mining pool operators eagerly install it. The fix of CVE-2018-17144 is the latest example of developers and pools streamlining deployment (versions: BTC 0.16.3 and BCHN 0.18.2), where the Slush pool collaborated with developers to deploy the upgrade before it was publicly released the day after discovery~\cite{CVE-2018-17144}. %Window of opportunity

However, for planned changes, the deployment must happen publicly and with enough time to review the proposal and implementation.
Back-room-like agreements between pools and developers will cause havoc in the community. The closest example of such behaviour has been seen in the Hong Kong Roundtable Consensus~\cite{hkrtc} and the New York Agreement~\cite{nya}, where prominent mining actors and central developers agreed to pursue a 2MB expansion fork on top of SegWit. The proposal was named Segwit2x, and the proponents held around 80\% of the network's hashing power. However, the proposal did not gain enough traction in the community and ended up being cancelled~\cite{segwit2x}.

Whether a change is a reduction, an expansion, or a bilateral fork is vital because reduction forks can be deployed with only a majority of miners. In contrast, expanding and bilateral forks require 100\% support from miners to prevent a chain split. Therefore, expanding and bilateral forks rely more on support from end-users to adopt the new chain, maintain its value, and pay fees. If a large portion of miners (e.g., 80\%) causes a chain split to deploy a change with low adoption from end-users (e.g., 20\%), then the new chain could lose its value, and miners would be incentivised to go back to the legacy chain to collect more fees. Therefore, the miners depend on user adoption to financially support the system, as much as users depend on miners for the system's security. With a reduction fork, the case is different because a majority of miners can deploy a change without causing a split. The rest of the network will have few choices except to accept the change.
If opposing miners and users wish to prevent or revert a reduction fork, they would have to gain control of the majority of hashing power or force a chain split by deploying a minority fork. %Therefore, if the Segwit2x proposal was a reduction fork, they could force the rest of the network to abide by their consensus change. However, as it was an expanding fork, they would rather detach from the legacy network.
% either my a minority reduction fork, expansion fork, or bilateral fork. 

%make another reduction fork to exclude blocks enforcing the new rules, if they can be identified. Alternatively the they would have to make an expanding or bilateral fork to revert the unwanted reduction fork. None of the alternatives are optimal as they require a chain split.

%Figure \ref{fig:power} is a high-level abstraction of how the actors in a blockchain look and illustrate the division of power. 

Controversial changes can be tedious to deploy, regardless of the fork type. Controversial proposals often lead the community to split in two and raise opposing and often irrational voices expressing FUD (fear, uncertainty, and death) or shill to represent all the advantages and fortune that can be made by deploying the change.
In these cases, the developers of a change must carefully use the deployment techniques for a change, optimally leading to deployment without a chain split or no deployment at all.
Miners choose whether they want to support the change or not. That decision heavily relies on seeing the direct benefit of that change and whether the users are willing to adopt and pay for the system's services after the change.

\subsection{RQ 1: Roles in governance}

The nodes running in a blockchain network are complex and connected in an {\tt m-n} fashion in the peer-to-peer network. The Wenn diagram in~\cref{fig:wenn} illustrates the complexity of the four roles an actor can take in a blockchain network.
These roles in ~\cref{fig:wenn} are abstractions based on the capabilities that an actor can have as a participant in the network. The purpose of the figure is to show that an actor or a blockchain node can come in many different shapes, mixing capabilities and multiple roles.
The diagram is mainly divided between full nodes and simple payment verification (SPV) nodes. A full node runs validation based on all consensus rules and needs all blockchain data to do so. On the other hand, SPV nodes run no or partial consensus validation.
The SPV nodes connect to full nodes in the network to ensure correctness of their state. It is possible to have a seed node, as shown in the figure. However, it is not common or useful to only store and relay blocks without consensus validation.
% Could write that other articles don't make this differentiation, but Im not sure what to cite.

We define the capabilities of the four abstracted roles in~\cref{fig:wenn} as follows: 1) Developers have access to all the components in the diagram but do not necessarily run any node. Developers can \textit{propose} changes to the consensus rules (\textit{constitution}) 2) Full nodes adopt the consensus rules proposed by the developers and must hold all blockchain data from the genesis block to enable full validation. By performing full validation, they \textit{judge} the correctness of proposed blocks from miners 3) Miners run mining operations, and \textit{enforce} the consensus rules upon users by deciding whether their transactions will be included in blocks. Miners often do not contain all blockchain data nor validate all consensus rules. Instead, they perform simple payment verification (SPV) - a partial validation of transactions and blocks. 4) End-users can be satisfied by running any wallet service. The end-users have the power to \textit{choose} which wallet they use, which connects to certain full nodes - ultimately choosing which \textit{constitution} to follow.

As the figure shows, a single node can represent one or many of these roles at the same time. \Cref{fig:topology} illustrates how the actors are connected in the Bitcoin network. The main takeaway from~\cref{fig:topology} is to show how actors can have different and multiple roles and how they are irregularly connected. It also demonstrates how consensus is maintained even though many nodes do not perform full validation.
Instead, nodes must eventually connect to a full node to ensure the validity of their state. Additionally, full nodes connect to each other to maintain consensus. The figure is an illustration and does not resemble the real network distribution in Bitcoin.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/wenn.png}
    \caption{Blockchain node Wenn diagram. The diagram illustrates the roles in consensus (RQ 1). Developers propose changes, full nodes adopt the changes to judge the validity of blocks and transactions, miners enforce consensus rules by generating blocks, and end-users can choose which consensus rules to abide by connecting to the full nodes in the network they prefer. The diagram includes simple payment verification (SPV), a method for nodes (e.g., end-users, miners, and validators) to perform partial verification without having to check every consensus rule or store the whole blockchain.}
    \label{fig:wenn}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/topology.png}
    \caption{The diagram illustrates an example of a heterogeneous blockchain network where actors connect dynamically and combine different roles. Everyone connects to a full node directly or indirectly. SPV nodes may not interconnect. Only rules validation or only serving blockchain data is not common. The topology of Bitcoin is complicated, and our purpose is to show this and that actors come in many shapes, mixing roles.}
    \label{fig:topology}
\end{figure}

One can argue that the development of some repositories, such as Bitcoin Core, is centralised~\cite{parkin2019senatorial,de2016invisible}. However, the developers can only change that specific implementation to \textit{propose} consensus rules. They cannot force anyone to use them. At the same time, the full nodes hold the consensus rules and \textit{judge} which chain their connected users will follow in case of a split. In contrast, miners cannot be expected to follow consensus rules entirely, as some will omit block and transaction validation to gain an advantage in the block-race~\cite{invalidBlocks}. In the end, miners decide the future of a blockchain, whether nodes will evolve in harmony or split into different blockchains.

Miners \textit{enforce} the consensus rules upon users by including transactions and producing blocks. Without miners, the blockchain will stop extending. The miners can deploy a reduction fork without causing a chain split by having majority adoption or 100\% miner adoption in expanding and bilateral forks. There will always be an economic incentive to avoid chain splits because the network will be perceived as more reliable if it stays consistent. In the end, users can \textit{choose} which wallet to use, which full nodes to connect to, which network they will be part of, and, therefore, which consensus rules to follow.

\begin{mybox}
\textbf{Summary of RQ 1:}
\textit{Which roles and actors can apply changes to consensus?}
\begin{enumerate}
  \item Developers \textit{propose} consensus rule changes.
  \item Full nodes \textit{judge} consensus rules by ensuring the validity of transactions and blocks.
  \item Miners \textit{enforce} the rules by choosing which transactions to include and generating blocks.
  \item End users \textit{choose} which full nodes they connect to, ultimately choosing which blockchain and corresponding consensus rules they like to use.
\end{enumerate}
\end{mybox}

%\subsection{Bitcoin governance overview} 
%\label{overview}

%TODO: Satoshi and Gavin were benevolent dictators. The 2013 fork resolution.


\subsection{RQ 2: The decision-making process of Bitcoin consensus governance} 
\label{keyEvents}

By using {\tt Matplotlib}~\cite{matplotlib} to make a graphical representation of signals related to consensus forks in BTC, we generated the graphs~\cref{fig:BTCevolutionLight} and~\cref{fig:BCHevolutionLight}, which include key governance events up until 2018 to highlight evolutionary decisions made in BTC's history. The y-axes represent the percentage of signalling blocks based on the latest 1000 blocks, and the x-axes show the time. %Solid lines show the signals retrieved from coinbase messages or the version bit field from blocks. The lines are dotted after activation to show that they no longer make a difference. The dashed lines at the top of \cref{fig:BTCevolutionLight} show the timing of successful deployments where those signals reached the required threshold of miner-activated strategies (precentage based activation) or were triggered by user-activation (flag day) or emergency-activation (urgent deployment). 
All the plots are retrieved from the BTC blockchain. At the same time, the graphs are separated to enhance readability, \cref{fig:BCHevolutionLight} only contain plots related to failed attempts to deploy blocksize increase. The graphs in \cref{fig:BTCevolutionLight} and \cref{fig:BCHevolutionLight} only include the deployment processes and events discussed in this section.
More detailed graphs are included in~\ref{signals} to show all on-chain activity.
%until 2022. \Cref{fig:BTCevolution} shows all the signals related to activated changes in BTC, including known activation timings in BTC. \Cref{fig:BCHevolution} shows all the BTC signals related to failed attempts of deploying increased block size combined with BCH flag day timings. Since the chain split, The BCH chain has not utilised signals in the deployment process. Instead, miners often signal which node implementation they support (e.g., BCHN)~\cite{cashNodes}. Some rule changes are not included in the graphs because it is impossible to state the exact activation time. That is because these deployments did not have an exact timing based on a signal, flag day/block height or chain split. Those are BTC 0.3.5, BTC 0.3.6, BTC 0.3.7, BTC 0.9.2, BTC 0.14.0 (CVE-2018-17144), BTC 0.16.3. and BCHN 0.18.2. Most of these changes were deployed through emergency-activation.

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figures/BTCSignalsNumbered.png}
    \caption{The graph illustrates key deployments in BTC. Solid lines depict the miners attempting to coordinate and enforce adopting new consensus rules by including signals in blocks. The changes activate based on a threshold, shown as dashed lines on the top. The included changes were mainly deployed using the miner-activated reduction fork (MARF) technique. After signals are faded/dotted after the point of activation to show that they no longer serve a purpose. One of the changes {\color{red}~\textit{BTC (fork) 0.14.0}} was a user-activated reduction fork, i.e., a flag day activated fork without on-chain coordination.}
    \label{fig:BTCevolutionLight}

    \centering
    \includegraphics[width=1\textwidth]{figures/BCHSignalsNumbered.png}
    \caption{The graph shows failed attempts to coordinate and enforce adopting new consensus rules for increased blocksize. Using a miner-activated expansion fork (MAEF) technique, the miners included block signals to show readiness. If the threshold was reached, those miners would have created a chain split. One of the attempts (BIP100) was particularly close to reaching the 75\% threshold.} 
    \label{fig:BCHevolutionLight}
\end{figure*}


Key governance events are identified by the red and bold labels in the text and~\cref{fig:BTCevolutionLight,,fig:BCHevolutionLight}. {\color{red}~\textbf{P2SH}}) In the early stages of Bitcoin, from late 2011 and early 2012, developers \textit{proposed} three conflicting proposals for pay-to-script-hash (P2SH) (BIP12, BIP16, and BIP17), influential Bitcoin developers stood behind each proposal. Miners attempted to \textit{enforce} the adoption using a simple MARF deployment technique (is-super-majority ISM) to coordinate an upgrade for the first time. The MARF technique was simple because the activation threshold was evaluated manually, and the timing was moved manually. In contrast to ISM, later deployments implemented a rolling window to activate automatically based on the threshold~\cite{self}.

The BIP12 proposal was at first discarded when a bug allowing unlimited recursion was discovered in the code. Afterwards, two conflicting proposals were created: BIP16 and BIP17. The conflicting proposals made the situation even more contentious. At that time, the operator (Tycho) of Bitcoin's biggest mining pool (Deepbit) represented roughly 1/3 of the hash power and the reluctant voice of opinion by being unwilling to support the and \textit{enforce} the \textit{proposal} before it gained more traction and technical guarantees, as seen in~\cref{tycho}. 

\begin{lstlisting}[style=quote, caption={Tycho 2012-01-25 Forum, ID: 61125}, label=tycho]
I would like to add something about one of the reasons why I don't want to be the FIRST to adopt P2SH: I don't like doing beta tests in a production environment. In last 2 days I already got 3 messages from Gavin about new bugs found in his implementation: one "minor bug" and one "major bug" ("one critical line was dropped in a merge and missed in my testing"). Also some coins were possibly destroyed in the process because a bug caused block fees to be lost.
\end{lstlisting}
%2012-01-25 BIP 16 / 17 in layman's terms 61125.html

%Also, you should note that I'll vote for /P2SH/ if considerable part of other miners will. It's not like I'm completely against it. My position is rather "Vote for doing it in a better way unless impossible" and not triggering the avalanche by voting myself first.
In the end, with more improvements to the BIP16 proposal, miner support, and influence from most of the Bitcoin Core developers, the miners coordinated to~\textit{enforce} BIP16 as the desired solution. The contention of deploying this feature and the manual change of the timing caused a delay in the deployment process, which led some full nodes to~\textit{enforce} the rule change too early, causing connected miners to get stuck.

The consensus mechanisms of the blockchain restricted the developer's decisions on the implementation and deployment of P2SH. The political view was that the change should be compatible with old nodes.
The rule changes were implemented as a hack-solution to achieve compatibility, making it a reduction fork.
Further, the deployment relied on majority adoption to avoid a chain split. The arbitrary coinbase message in blocks was used as a governmental instrument to measure and reach the adoption threshold before activation.

{\color{red}~\textbf{BIP16}}) The signal for BIP16 stayed active for a few years after the activation of P2SH. The signal does not matter and stayed active because it was not removed from the code before 2015~\cite{6203}. After activation, the blue line signalling BIP16 shows traces of miners turning off the flag manually as it goes down before going up again with major releases of Bitcoin Core, which by default included the signal in the coinbase message.
In later versions from and including BTC 0.12.1 - "CHECKSEQUENCEVERIFY" \textbf{CSV)} the activation signals were configured to cease as soon as they served their purpose, seen as an immediate drop in support after activation.

{\color{red}~\textbf{Database}}) The Bitcoin network experienced an accidental chain split caused by an unintended non-deterministic expansion fork when switching from Berkeley DB to Level DB in BTC 0.8.0 \cite{BIP-0050}. One could say that the full nodes and miners were split in two, judging and enforcing different constitutions. The end-users and miners would follow the chain judged as valid by the full nodes they were running or connected to. As shown in~\cref{rollbackIRC}, developers (Luke-Jr, sipa, jgarzik, and gavinandresen) and pool operators (Eleuthria and doublec) coordinated a rollback of Bitcoin to let the nodes reorganise to the legacy chain.
This emergency response shows a case where the centralisation tendencies in the developer team and pools streamlined the governance process.

\begin{lstlisting}[style=quote, caption={Developers: Luke-Jr, sipa, jgarzik, and gavinandresen. Pool operators: Eleuthria and doublec 2013-03-12 IRC: \#bitcoin-dev}, label=rollbackIRC]
<Luke-Jr> gavinandresen: sipa: jgarzik: can we get a consensus on recommendation for miners to downgrade? (...)
<Eleuthria> I can single handedly put 0.7 back to the majority hash power
<Eleuthria> I just need confirmation that thats what should be done (...)
<sipa> Eleuthria: imho, that is was you should do, but we should have consensus first (...)
<jgarzik> sipa, Eleuthria: ACK on preferring 0.7 chain, for the moment (...)
<gavinandresen> Eleuthria: if you can cleanly get us back on the 0.7 chain, ACK from here, too (...)
<Eleuthria> alright (...)
<doublec> ok, rolling back to 0.7.2
\end{lstlisting}

BTC's consensus mechanisms and technical landscape steered the community toward a rollback to the legacy, flawed implementation. Since BTC 0.8.0 was a (non-deterministic) expansion fork, the network would require all miners to upgrade and discard the legacy chain fork. On the other hand, only a majority had to mine on the legacy chain to discard the new chain. Additionally, many end-users still relied on legacy implementations, such as Mt.Gox, the largest exchange at the time. If the community choose to proceed with BTC 0.8.0, it would be a long-lasting inconsistency with service outages. Only a rollback enforced by an emergency-activated reduction fork (EARF) could quickly gather the community on one chain. The later patch (BTC 0.8.1) was created as an uncontroversial change to fix the bug permanently and deployed through user-activation (flag day) since resolving the bug was more important than keeping the network consistent with unpatched nodes at that point. %The patch gave node operators reasonable time to upgrade through a flag day.

{\color{red}~\textbf{DER}}) The deployment of BIP66 implemented in BTC 0.10.0 - "Strict DER signatures" demonstrates full nodes passing judgment on misbehaving miners. The incident occurred during the activation in July 2015 without notable traces in the graph. Regarding governance, roughly 50\% of the miners were not performing full validation according to new rules, enforced old rules as they had signalled for and generated competing forks. The full nodes noticed this and rejected those blocks, and the full node validated chain prevailed. The quote in~\cite{SPVMining} emphasises the risk of mining without validation.

\begin{lstlisting}[style=quote, caption={Bitcoin.org \cite{invalidBlocks}}, label=SPVMining]
Note that the roughly 50% of the network that was SPV mining had explicitly indicated that they would enforce the BIP66 rules. By not doing so, several large miners have lost over $50,000 dollars worth of mining income so far. 
\end{lstlisting}
%https://bitcoin.org/en/alert/2015-07-04-spv-mining#solution

{\color{red}~\textbf{SegWit}}) The most contentious consensus rule change of Bitcoin and any blockchain so far is the deployment of SegWit in August 2017. In the beginning, the pink line in~\cref{fig:BTCevolutionLight} (year: 2017) shows the struggle to reach the required 95\% threshold. This struggle is often referred to as an attempt to veto the deployment of SegWit.
Many SegWit proponents were determined to force through the upgrade with a user-activated reduction fork (UARF) and set a flag day to exclude non-signalling nodes on 2017-08-01. They gained support from the SegWit2x community, who intended to enforce SegWit signalling triggered by a 80\% threshold.
The SegWit2x community also intended to increase the blocksize of Bitcoin later, albeit they were not successful. The SegWit2x community adopted BIP91 to reduce the evaluation window and reached its threshold on 2017-07-20.
The original 95\% threshold was reached on 2017-08-08, and the planned miner-activated reduction fork (MARF) deployment technique then activated SegWit after a grace time of 2016 blocks on 2017-08-24. 

The point of highlighting the deployment process of SegWit is to show how external (SegWit2x/BIP91) and anonymous (BIP148) developers enabled miners to enforce the upgrade using a reduced threshold, flag day activation, and exclusion against the advice of core developers behind the original proposal (BIP141, BIP143 and BIP147). As the quotes in~\cref{sipaUASF,maxwellUASF} emphasise, the miners went through with a user-activated reduction fork (UARF - noted as UASF or BIP148 in the quotes) even though it was discouraged by developers from the centralised core team and increased the risk of a chain split.

\begin{lstlisting}[style=quote, caption={Sipa 2017-05-17 Github: Pull 10417}, label=sipaUASF]
I believe there is widespread support for SegWit, and I sure as hell hope it activates at some point in time. Unsure if you're aware, but I'm the primary author of the SegWit proposal and patches. However, I don't think there is a rush, and BIP148 seems an unnecessarily risky way to bring that about.
\end{lstlisting}

\begin{lstlisting}[style=quote, caption={Gregory Maxwell 2017-04-05 Email: \#bitcoin-dev}, label=maxwellUASF]
I do not support the BIP148 UASF for some of the same reasons that I do support segwit:  Bitcoin is valuable in part because it has high security and stability, segwit was carefully designed to support and amplify that engineering integrity that people can count on now and into the future.
\end{lstlisting}

A minority introduced the UARF deployment technique as a governmental instrument to persuade the sceptics to adopt SegWit. The UARF worked such that patched nodes would discard blocks that were not signalling support for SegWit. Therefore, the proponents demonstrated a willingness to bet on Bitcoin's economic future to ensure SegWit adoption with two possible outcomes. First, a majority of nodes discard non-signalling nodes, and the non-signalling nodes will be denied block rewards. Second, a minority of nodes discard non-signalling blocks, making a chain split, causing the legacy network to lose a significant portion of its users and miners, leading to network disruption and economic instability. The more users and miners enforce signalling, the more it impacts non-signalling miners.

The graph in~\cref{fig:BCHevolutionLight} depicts several failed attempts to activate increased blocksize with miner-activated expansion forks (MAEFs) in Bitcoin between 2015 and 2018. {\color{red}~\textbf{BIP100}}) The signal with the highest support was BIP100 which reached support higher than 60\%. However, the activation threshold of 75\% was never reached. This expansion fork would have split the chain in two if it were to happen with less than 100\%, and end-users and miners would follow one of them depending on which constitution they like, judged by the full nodes they chose to run or connect to. It is also worth noting that each of these proposals was backed by at least one highly influential developer, the successor of Satoshi Nakamoto: Gavin Andresen.
However, his influence did not convince a significant majority to adopt larger blocks. The quote in~\cref{ballsyAndresen} indicates lead maintainer Andresen's failed assumption of having actual decision-making power as a {\tt benevolent dictator}.

\begin{lstlisting}[style=quote, caption={Gavin Andresen 2015-04-18 \cite{ballsyAndresen}}, label=ballsyAndresen]
That may be what has to happen with the blocksize, frankly. I may just have to throw my weight around and say: This is the way its gonna be and if you don't like it, go find another project.
\end{lstlisting}
%28:30
%https://www.youtube.com/watch?v=RIafZXRDH7w&t=1672s



BCH was deployed as an alternative to BTC's SegWit user-activated reduction fork in August 2017. The deployment was commenced using a user-activated bilateral fork technique (UABF). The deployment classifies as user-activated because it relied on flag day activation without on-chain coordination to reach a certain threshold of support before activation. Additionally, the fork would activate using a flag day regardless of network adoption, thus prioritising the features of BCH before the consistency of the network. BCH's increase in block size is an expansion fork by itself. If BCH was deployed as a plain expansion fork, it would still accept SegWit blocks. Additional changes were needed since the fork was likely to be deployed by a minority. Therefore, BCH's deployment implementation required the first block in BCH to be larger than 1MB, causing a conflict between the legacy and the new chain. This conflict makes BCH a bilateral fork rather than an expansion fork to ensure a permanent chain split at the activation time. The deployment of BCH demonstrates another connection between the governance of the infrastructure and governance by the infrastructure.

After the forking and deployment of BCH, the remaining planned upgrades in BCH have all been deployed using flag-day-based user-activated strategies. BCH is being operated with several node implementations~\cite{full-nodes}, and Bitcoin Cash Node (BCHN) is one of them. Thus, a successful and consistent deployment relies on the developers maintaining those implementations to agree on the path forward and the miners to harmonise the changes.
There are two events where BCH has experienced disruptions causing permanent chain splits. One was in the event of splitting off Bitcoin SV (November 2018), and the other one was splitting off Bitcoin ABC (November 2020). These events further suggest that user-activated strategies value new functionality over the consistency of the network and the blockchain.

\begin{figure*}
    \includegraphics[width=1\linewidth]{figures/decision-making.png}
\end{figure*}

\begin{mybox}
  \textbf{Summary of RQ 2:}
  \textit{What is the decision-making process for consensus changes?}
  \begin{itemize}
    \item The community usually coordinates to implement support for changes before they are deployed, either by on-chain coordination or flag-day-based activation.
    \item Developers decide whether a change will be included in their implementation.
    \item Users, developers, miners and validators that will not accept a change can choose not to utilise an upgrade and fork to a new code base and chain split if necessary.
    \item Mining pool operators can adopt changes on behalf of miners in their pool. Miners that disagree can change the pool or mine independently.
    \item Full nodes can adopt changes on behalf of connected users. Users who disagree can connect to different full nodes. For instance, by using a different wallet.
    \item Emergency upgrades ignore the conventional processes and should roll back as quickly as possible. A swift rollback can be enabled by coordinated developer teams and pools that can control connected miners.
  \end{itemize}
  
\end{mybox}

\subsection{RQ 3: Roles and decision-making power distribution}

The consolidation of results of the social and political aspects of the governance reveals the process and balance of power deciding the evolutionary path for a decentralised distributed ledger as illustrated in~\cref{fig:power}.
The figure shows that the consensus rules or the implementation resemble the system's constitution. Developers act as a council and can propose changes, which will be enforced in practice if the miners choose to do so. Full nodes are the only actors who fully validate the blockchain according to the consensus rules and the complete history of the ledger. Hence, full nodes act as judges in the blockchain.

The end-users can choose whatever blockchain they like, depending on their preferred consensus rules. In practice, they do that by running a full node-powered wallet or, more commonly, a simple payment verification (SPV) wallet connected to full nodes running a specific implementation. Miners enforce the consensus rules by including transactions in blocks and broadcasting them on the network. If a miner violates the rules of the end-user's full nodes, their blocks and transactions will not be accepted. 

Anyone can participate in any or all of the roles if they like. If the constitution is unsatisfactory, anyone may fork off and change it. However, any blockchain holds its value in participation and adoption, and all the actors will generally benefit from collaborating. Whether a rule change is worth deploying is a tradeoff between the impact of the new functionality and the impact on the network's consistency. The miners also benefit from choosing the path supported by the community and the economic majority, which is viable for the system's stability and long-term efficacy.


\begin{figure}
  \centering
  \includegraphics[height=\linewidth]{figures/power.png}
  \caption{Blockchain governance: roles and decision-making power distribution. The pattern closely resembles the tripartite system's division and balance of power~\cite{tripartite}. Except that anyone can participate in any and as many roles as they want. The miners can enable consensus change. However, they are incentivised to do so only with significant support from the community, including other roles.}
  \label{fig:power}
\end{figure}

The deployment techniques and historical observations related to Bitcoin demonstrate a flat and decentralised decision-making power structure among miners within the blockchain. As highlighted in~\cref{fig:power}, anyone can act as a developer and write code, but \textbf{it ultimately falls upon the miners to adopt consensus changes}.
Bitcoin operates neither as an oligarchy nor a democracy; rather, it functions through consensus, driven by miners and governed by the longest valid chain rule. \textbf{The concept of validity remains subjective, allowing each individual to choose their preferred approach.} However, consistency is crucial, and a cryptocurrency's value hinges on its usage and adoption.
Additionally, security in Proof of Work (PoW) blockchains relies on the total hash power and its distribution across the network. Therefore, it might be desirable to avoid controversial forks or reconcile with the majority fork in case of a chain split.

A limitation of Bitcoin's evolution governance structure is that few quality assurance indicators allow miners, full nodes and users to assess the security of a change proposed by developers. We urge these actors to demand more insights into the amount of testing and review that has gone into changes before adopting them. Although such processes exist, they are often not well communicated. For instance,~\cref{ACK} shows a reviewer's approval of the code for a reduction fork (BIP66~\cite{BIP-0066}). In total, there are six participants commenting on the proposed code and ten comments on the proposal. Anyone who is not an expert in cryptography would have to trust the statements of these participants in this thread without more insights into the extent of assurances tied to the BIP66 consensus change.

\begin{lstlisting}[style=quote, caption={Laanwj 2015-01-28 Github: Pull 5713}, label=ACK]
tested ACK. Verified that the deployment behavior as mentioned in BIP66 is indeed what is enforced.
\end{lstlisting}

\begin{lstlisting}[style=quote, caption={2023-10-13 Peter Todd and Dave Weisberger \cite{drivechain}}, label=drivechain]
<Peter Todd> If we have a UASF that doesn't have overwhelming support, which is what would happen with drivechains if this goes badly, suddenly bitcoin forks and very bad stuff happen where one exchange is simply not on the same bitcoin as another exchange, yet they still have the same ticker price. (...)
<Dave Weisberger> I'm going directly to the miners, and I'm making a case for why they need to adopt drivechain, and I'm selling them on the benefits of it, and frankly I don't care what anyone else's views are because it is the miners at the end of the day that I have to convince. If the community has a problem with that, then what can they do to stop them?
<Peter Todd> What you are telling miners here is that this is going to be a shitshow. And if you go through this and add all this uncertainty to Bitcoin. Ultimately, you are probably either to just reduce the price in general, or you will go have a UASF to undo drivechains and that is a huge mess. (...) It is a much bigger mess than just doing nothing. (...)
\end{lstlisting}
%https://www.youtube.com/watch?v=YM_b6q7l0H4&t=14s
%2:23 - 2:25:05

\begin{mybox}
  \textbf{Summary of RQ 3:}
  \textit{How is decision-making power distributed among the different roles in consensus evolution?}
  
  As envisaged, there is not a single entity or role that single-handedly holds the power to change consensus. Developers, users, and full nodes depend on each other for a blockchain to serve its purpose. The blockchain mechanisms regarding consensus change predict two outcomes: either everyone agrees to act in the way and build a single chain, or the blockchain and the community will split. The success of a fork depends on the grade of adoption by users, developers, full nodes and miners.
\end{mybox}



==> sections/results/resultsPreamble.old.tex <==
% This section was moved into RQ3

\subsection{The relationship between governance process and the level of controversy of a change}
\label{governance}

The analytical codes related to the social/political category (\cref{fig:codesCategories}) depict how the governance process relies on the debates and arguments concerning the change.
A non-contested change with low controversy requires low effort in convincing the community and scheduling deployment.
Centralisation tendencies in development and mining operations can streamline the deployment of non-contested changes. Changes that can be deployed most quickly are related to fixing an immediate issue in the blockchain. In that case, the developers are in a hurry to implement a solution while miners and mining pool operators eagerly install it. The fix of CVE-2018-17144 is the latest example of developers and pools streamlining deployment (versions: BTC 0.16.3 and BCHN 0.18.2), where the Slush pool collaborated with developers to deploy the upgrade before they released the code the day after discovery~\cite{CVE-2018-17144}. %Window of opportunity

However, for planned changes, the deployment must happen publicly and with enough time to review the proposal and implementation. Back-room-like agreements between pools and developers will cause havoc in the community. The closest example of such behaviour has been seen in the Hong Kong Roundtable Consensus~\cite{hkrtc}, and New York Agreement \cite{nya}, where prominent mining actors and central developers agreed to pursue a 2MB expansion fork on top of SegWit. The proposal was named Segwit2x, and the proponents held around 80\% of the network's hashing power. However, the proposal did not gain enough traction in the community and ended up being cancelled~\cite{segwit2x}.

Whether a change is a reduction, an expansion, or a bilateral fork is vital because reduction forks can be deployed with only a majority of miners. In contrast, expanding and bilateral forks require 100\% support from miners to prevent a chain split. Additionally, services like wallets and exchanges might require changes to support expanding and bilateral forks. Therefore, expanding and bilateral forks rely more on support from end-users to adopt the new chain, maintain its value, and pay fees. If miners force the activation of a controversial proposal without users' support, the cryptocurrency could depreciate. Therefore, the miners depend on user adoption to financially support the system, as much as users depend on miners for the system's security. With a reduction fork, the case is different because a majority of miners can deploy a change without causing a split. If opposing miners and users wish to prevent or revert a reduction fork, they would have to gain control of the majority of hashing power or force a chain split by deploying a minority fork. ~\cref{drivechain} shows Bitcoin Core developer Peter Todd sharing his view on why forcing changes is generally bad.

%Therefore, if the Segwit2x proposal was a reduction fork, they could force the rest of the network to abide by their consensus change. However, as it was an expanding fork, they would rather detach from the legacy network.
% either my a minority reduction fork, expansion fork, or bilateral fork. 

%make another reduction fork to exclude blocks enforcing the new rules, if they can be identified. Alternatively the they would have to make an expanding or bilateral fork to revert the unwanted reduction fork. None of the alternatives are optimal as they require a chain split.

%Figure \ref{fig:power} is a high-level abstraction of how the actors in a blockchain look and illustrate the division of power. 


\begin{lstlisting}[style=quote, caption={2023-10-13 Peter Todd and Dave Weisberger \cite{drivechain}}, label=drivechain]
<Peter Todd> If we have a UASF that doesn't have overwhelming support, which is what would happen with drivechains if this goes badly, suddenly bitcoin forks and very bad stuff happen where one exchange is simply not on the same bitcoin as another exchange, yet they still have the same ticker price. (...)
<Dave Weisberger> I'm going directly to the miners, and I'm making the case for why they need to adopt drivechain, and I'm selling them on the benefits of it, and frankly, I don't care what anyone else's views are because it is the miners at the end of the day that I have to convince. If the community has a problem with that, then what can they do to stop them?
<Peter Todd> What you are telling miners here is that this is going to be a shitshow, and if you go through this and add all this uncertainty to Bitcoin. Ultimately, you are probably either to just reduce the price in general, or you will go have a UASF to undo drivechains and that is a huge mess. (...) It is a much bigger mess than just doing nothing. (...)
\end{lstlisting}
%https://www.youtube.com/watch?v=YM_b6q7l0H4&t=14s
%2:23 - 2:25:05

Controversial changes can be tedious to deploy, regardless of the fork type. Controversial proposals often lead the community to split in two and raise opposing and often irrational voices expressing FUD (fear, uncertainty, and death) or shill to represent all the advantages and fortune that can be made by deploying the change. In these cases, the developers of a change must carefully use the deployment techniques for a change, optimally leading to deployment without a chain split or no deployment at all. Miners choose whether they want to support the change or not. That decision heavily relies on seeing the direct benefit of that change and whether the users are willing to adopt and pay for the system's services after the change.


==> tables/deploymentTechniques.tex <==
\begin{table*}
    \footnotesize
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    % Most reasonable to include the release for the change since the blockcheight and timing isnt always certain
    % Include commit hash because different sources are inconsistent
    \caption{Deployment techniques. The notations indicate whether the features are required to reduce the chain split risk and the impact of a chain split: \textbf{Bold: Essential}, \textit{Itallic: Useful}, -: Insignificant. The abbrevations are: Miner-activated (MA), user-activated (UA), emergency-activated (EA), reduction fork (RF), expansion-fork (EF), bilateral fork (BF), and super-majority (SM) \cite{self}}
    \centering
    \begin{tabular}{llllllllll}%    \begin{tabular}{p{2cm}|p{1.3cm}|p{2cm}|p{3cm}|p{3cm}}
    \textbf{Deployment} & \textbf{Fork} & \textbf{Chain} & \textbf{Parallel} & \textbf{Standard} & \textbf{Signal} & \textbf{Inclusive} & \textbf{Threshold} & \textbf{Trigger} & \textbf{Example consenus} \\
    \textbf{strategy} & \textbf{type} & \textbf{split risk} & & & & &  & & \textbf{rule change} \\
    \hline
    MA & RF & Low & \textit{Yes} & \textbf{Yes} & \textbf{Yes} & \textit{Exclusive} & \textbf{SM} & \textbf{Dynamic} & Reduce max blocksize \\
    \hline

    MA & EF & High & \textit{Yes} & \textit{Yes} & \textbf{Yes} & \textit{Exclusive} & \textbf{100\%} & \textbf{Dynamic} & Increase max blocksize \\
    \hline

    MA & BF & High & \textit{Yes} & \textit{Yes} & \textbf{Yes} & - & \textbf{100\%} & \textbf{Dynamic} & Increase max blocksize \& \\
    & & & & & & & & & set min blocksize \textgreater legacy blocksize \\
    \hline

    UA & RF & Medium & \textit{Yes} & \textbf{Yes} & \textit{Yes} & \textbf{Exclusive} & \textbf{None} & \textbf{Static} & Reduce max blocksize \\
    \hline

    UA & EF & High & \textit{Yes} & \textit{Yes} & \textit{Yes} & \textbf{Exclusive} & \textbf{None} & \textbf{Static} & Increase max blocksize \\
    \hline
    
    UA & BF & High & \textit{Yes} & \textit{Yes} & \textit{Yes} & - & \textbf{None} & \textbf{Static} & Increase max blocksize \& \\
    & & & & & & & & & set min blocksize \textgreater legacy blocksize \\
    \hline

    EA & RF & Medium & \textit{Yes} & - & - & \textit{Inclusive} & \textbf{None} & \textbf{Instant} & Reduce max blocksize \\
    \hline

    EA & EF & High & \textit{Yes} & - & - & \textbf{Exclusive} & \textbf{None} & \textbf{Instant} & Increase max blocksize \\
    \hline

    EA & BF & High & \textit{Yes} & - & - & - & \textbf{None} & \textbf{Instant} & Increase max blocksize \& \\
    & & & & & & & & & set min blocksize \textgreater legacy blocksize \\
    \hline

    \end{tabular}


    \label{tab:forkTypes}
\end{table*}

==> tables/deployments.tex <==
%UASF has to be exlusive?
% SHOW START, END, PERIOD?
\begin{table}
    \tableFontSizeSmall
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    % Most reasonable to include the release for the change since the blockcheight and timing isnt always certain
    % Include commit hash because different sources are inconsistent
    %    \centering
    %\resizebox{\textwidth}{!}{
    %\renewcommand{\arraystretch}{1.5} % Default value: 1
    \begin{tabular}{lllllllllll}
    \textbf{V} & \textbf{Consensus change} & \textbf{Deployment} & \textbf{Fork} & \textbf{Chain} & \textbf{Signal} & \textbf{Threshold} & \textbf{Trigger} & \textbf{Inclusive} & \textbf{Standard} & \textbf{Parallel}\\
    & & \textbf{Strategy} & \textbf{Type} & \textbf{split risk} & & & & & & \\
    \hline
    BTC & Time based locking & UA & RF & Medium & None & None & BH & Inclusive & No & Yes \\
    0.1.6 & nLockTime & & & & & & & & & \\
    \hline
    BTC & CVE-2010-5137 \& & EA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.3.5 & CVE-2010-5141 & & & & & & & & & \\
    \hline
    
    BTC & Disable/enable opcodes & EA & EF \& RF & High & None & None & Instant & Inclusive & No & Yes \\
    0.3.6 & & & \textit{hybrid} & & & & & & & \\
    \hline

    BTC & Separate scriptSig \&  & EA & EF \& RF & High & None & None & Instant & Inclusive & No & Yes \\
    0.3.7 & scriptPubKey & & \textit{hybrid} & & & & & & & \\
    \hline

    BTC & Output-value-overflow  & EA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.3.10 & CVE-2010-5139 & & & & & & & & & \\
    \hline
    
    BTC & 20 000-signature operation & UA & RF & Medium & None & None & BH & Inclusive & No & Yes \\
    0.3.12 & limit \& 1 MB blocksize & & & & & & & & \\
    \hline

    BTC & BIP30: Duplicate transactions & MA & RF & Low & Offchain & \textgreater 50\% & FD & Inclusive & No & Yes \\
    0.6.0 & CVE-2012-1909 & & & & agreement & & & & \\
    
    % / awareness
    
    \hline
    BTC & BIP16: Pay-to-script-hash & MA & RF & Low & Coinbase & 55\% & FD & Inclusive & No & Yes \\
    0.6.0 & & & & & vote & & & & & \\
    
    \hline
    BTC & BIP34: Include block height & MA & RF & Low & VersionBits & 75\%/95\% & DH & Exclusive & No & No \\
    0.7.0 & in coinbase & & & & & & & & & \\
    
    \hline
    BTC & BIP50: Migrate from & UA & EF \textit{non-} & High & None & None & Instant & Inclusive & No & Yes \\
    0.8.0 & Berkeley DB to LevelDB & & \textit{deterministic} & & & & & & & \\  
    \hline

    BTC & BIP50: Rollback & EA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.7.0 & & & & & & & & & & \\
    \hline
    
    BTC & BIP50: Database lock limit \& & UA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.8.1 & Max TxID limit & & \textit{temporarily} & & & & & & & \\
    \hline

    BTC & BIP50: Relax database lock & UA & EF & High & None & None & FD & Inclusive & No & Yes \\
    0.8.1 & limit \& Max TxID limit & & & & & & & & & \\
    \hline

    BTC & BIP42: 21 million supply & UA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.9.2 & & & & & & & & & & \\
    \hline

    BTC & BIP66: Strict DER signature & MA & RF & Low & VersionBits & 75\%/95\% & DH & Inclusive & Yes & No \\
    0.10.0 & & & & & & & & & & \\
    \hline

    %ERF??
    BTC & BIP65: Check lock time verify & MA & RF & Low & VersionBits & 75\%/95\% & DH & Inclusive & No & No \\ 
    0.11.2 & & & & & & & & & & \\
    % nVersion tx
    \hline

    %0.11A (XT) & BIP-101 & & & & & & & & \\

    BTC & BIP68, BIP112, BIP113: & MA & RF & Low & VersionBits & 95\% & DH & Inclusive & No & Yes \\
    0.12.1 & Check sequence verify & & & & & & & & & \\
    % script verification flag
    \hline

    %\hline
    %0.12.1 (classic) & BIP-102 & MAEF & High & VersionBits & 95\% & DH & Inclusive & No & Yes \\
    %& & Miner activated & & & & & &\\
    
    BTC & BIP141, BIP143, BIP146: & MA & RF & Low & VersionBits & 95\% & DH & Inclusive & Yes & Yes \\
    0.13.1 & Segregated Witness & & & & service bits & & & & & \\
    % script verification flag     
    
    \hline
    BTC & CVE-2018-17144 & UA & EF & High & None & None & Instant & Inclusive & No & Yes \\
    0.14.0 & & & & & & & & & & \\
    
    \hline
    BTC* & BIP148: Segregated Witness & UA & RF & Medium & VersionBits & None & FD & Exclusive & Yes & Yes \\
    0.14.0 & & & & & & & & \textit{temporarily} & & \\
    % script verification flag,  service bits p2p

    \hline
    BTC* & SegWit2x/BIP91: & MA & RF & Low & VersionBits & 80\% & DH & Inclusive & Yes & Yes \\
    0.14.1 & Segregated Witness & & & & & & & & & \\ % service bits p2p script verification flag 
    
    %\hline
    %0.14.1 Core & BIP91: Segregated Witness & MA & RF & Low & VersionBits & 80\% & DH & Exclusive & Yes & Yes \\
    %(forked) & & & & & & & & & & \\ %  service bits p2p script verification flag
    
    \hline
    BCHN & Block size fork & UA & BF & High & None & None & FD & Exclusive & No & Yes \\
    0.14.5 & & & & & & & & & & \\
    %Service bits
    
    \hline
    BCHN & LOW\_S \& NULLFAIL \& & UA & EF \& RF & High & None & None & FD & Inclusive & Yes & Yes \\
    0.16.0 & difficulty adjustment & & \textit{hybrid} & & & & & & & \\
    
    \hline
    BCHN & Block size increase \& & UA & EF & High & None & None & FD & Inclusive & No & Yes \\
    0.17.0 & enable opcodes & & & & & & & & & \\
    
    \hline
    BCHN & Various rule changes & UA & EF \& RF & High & None & None & FD & Inclusive & No & Yes \\
    0.18.0 & & & \textit{hybrid} & & & & & & & \\

    \hline
    BCHN & Fix CVE-2018-17144 & EA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.18.2 & & & & & & & & & & \\

    \hline
    BTC & Fix CVE-2018-17144 & EA & RF & Medium & None & None & Instant & Inclusive & No & Yes \\
    0.16.3 & & & & & & & & & & \\
    
    \hline
    BCHN & Schnorr signatures \& & UA & EF & High & None & None & FD & Inclusive & No & Yes \\
    0.19.0 & SegWit recovery & & & & & & & & & \\
    
    \hline
    BCHN & Schnorr signatures for & UA & EF \& RF & High & None & None & FD & Inclusive & No & Yes \\
    0.19.12 & multisig \& script attributes & & \textit{hybrid} & & & & & & & \\
    
    \hline
    BCHN & SigChecks \& & UA & EF & High & None & None & FD & Inclusive & No & Yes \\
    0.21.0 & Reversebytes opcode & & & & & & & & & \\
    
    \hline
    BCHN & ASERT Difficulty algorithm & UA & BF & High & None & None & FD & Inclusive & No & Yes \\
    22.0.0 & & & & & & & & & & \\
    \hline

    BCHN & Lift transaction chain limit \& & UA & EF & High & None & None & FD & Inclusive & No & Yes \\
    23.0.0 & Multiple OP\_RETURN outputs & & & & & & & & & \\
    \hline

    BTC & BIP341, BIP342, BIP343: & MA & RF & Low & VersionBits & 90\% & DH & Inclusive & Yes & Yes \\
    0.21.1 & Taproot & & & & & & & & & \\
    %script verification flag ,  min height    
    \hline
    
    BCHN & CHIP-2021-03 & UA & EF & High & None & None & FD & Inclusive & No & Yes \\
    24.0.0 & CHIP 2021-02 & & & & & & & & & \\
    \hline

    %perfective: Increase script maintainability
    % corrective: malleability
    % Adaptive: lightning, blocksize
    % Preventive: Bit32 microsoft
    
    \end{tabular}
        \caption{Deployed rule changes in BTC and BCH. Triggers: BH = Block height, FD = Flagday, and DH = Dynamic height.}
        \label{tab:deploymentTechniques}
    \end{table}

    %Versions marked (*) are forks outisde the main repository. 


==> tables/lessons.tex <==
\begin{table}
    \tableFontSizeSmall
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %    \centering
    \begin{tabular}{lllll}
    \textbf{ID} & \textbf{Lesson} & \textbf{Impacted features} & \textbf{Error categories} & \textbf{Negatvely affected versions} \\
    \hline
    
    L1 & Missing transformation assurance & Fork type & RB Mistake & BTC 0.8.0, BTC 0.14.0, BCHN 0.17.0 \\ % Missclassification
    \hline
    L2 & Improper reorganization & - & Lapse, KB Mistake & BTC 0.3.10, Before BTC 0.8.0, BTC 0.8.0 \\ % Deleting the old blockchain was a lapse. The implementation was not good to handle (KB)
    \hline
    L3 & Improper human interference & Trigger & Lapse, RB mistake, KB mistake & BTC 0.6.0 \\ % Gavin made a bad assumption, the miners didnt know or forgot
    \hline
    L4 & Too high thresholds & Threshold, inclusive \& & RB Mistake & BTC 0.13.1 \\ % We thought high thresholds were good
    & & deployment strategy & & \\
    \hline
    L5 & Deplyoing 'irreversible' changes & Fork type & KB Mistake & BTC 0.3.12 \\ % RB?
    \hline
    L6 & Not prepared for forward & Fork type, standard \& & KB Mistake & BTC 0.7.0, BTC 0.10.0, BTC 0.11.2 \\ % Rule base?
    & compatibility & parallelism & & \\
    \hline
    L7 & Lacking knowledge regarding & Signal & KB Mistake & - \\ % Rule base? KB mistake if it wasn't considered
    & network dynamics & & & \\
    \hline
    L8 & Insufficient damage control & - & KB Mistake & BTC 0.8.0 \\ %??
    \hline
    L9 & Improper miner incentives & - & Routine violation, Exceptional violation & BTC 0.10.0 \\ 
    & to enforce new rules & & & \\
    \hline
    L10 & Insufficient developer incentices & - & Routine violation & BTC 0.8.0, BTC 0.14.0, BCHN 0.17.0 \\
    & to review the code & & & \\
    \hline 
\end{tabular}
\caption{Lessons learned, impacted features, corresponding error categories and impacted Bitcoin versions.}
\label{tab:lessons}
\end{table}
